Deep Symbolic Regression for Recurrent Sequences

Symbolic regression, i.e. predicting a function from the observation of its values, is well-known to be a challenging task. In this paper, we train Transformers to infer the function or recurrence relation underlying sequences of integers or floats, a typical task in human IQ tests which has hardly been tackled in the machine learning literature. We evaluate our integer model on a subset of OEIS sequences, and show that it outperforms built-in Mathematica functions for recurrence prediction. We also demonstrate that our float model is able to yield informative approximations of out-of-vocabulary functions and constants, e.g. $\operatorname{bessel0}(x)\approx \frac{\sin(x)+\cos(x)}{\sqrt{\pi x}}$ and $1.644934\approx \pi^2/6$. An interactive demonstration of our models is provided at https://symbolicregression.metademolab.com.

==> acknowledgements.tex <==
\section*{Acknowledgements}

We thank Florent Krzakala for introducing us to feedback alignment, and we thank
him and Lenka Zdeborov\'a for organising the Les Houches 2020 workshop on
Statistical Physics and Machine Learning where this work was initiated. We thank
Florent Krzakala, Giulio Biroli, Charlotte Frenkel, Julien Launay, Martin
Lefebvre, Leonardo Petrini, Iacopo Poli, Levent Sagun and Mihiel Straat for
helpful discussions. MR acknowledges funding from the French Agence Nationale de la Recherche under grant ANR-19-P3IA-0001 PRAIRIE. SD acknowledges funding from PRAIRIE for a visit to Trieste
to collaborate on this project. RO acknowledges funding from the Region
Ile-de-France.


==> removed.tex <==
\section{Modelling stochasticity}

We now show that our model can be trained to predict the exact functional form of the stochastic noise. The key ingredient to do so is to introduce a random variable $\xi\sim\mathcal{N}(0,1)$ as a leaf in our mathematical trees during training, which is sampled with a probability $\pi_{train}$. The mean and variance of the noise will naturally be varied by addition or multiplication with constant leaves (e.g. $2+3\xi$), and can become time-dependent (e.g. $n^2\xi$) or scale-dependent (e.g. $u_{n}\xi$). 

As test time, we want to know if our model has captured the correct expression, for example $u_{n+1} = u_n + n^2\xi$. To assess this, we again use next-term prediction, removing the stochasticity on the extrapolated points.

\paragraph{Results}

In Tab.~\ref{tab:random-leaves}, we show that by adding random leaves at training time, we enable the model to model simple stochastic expressions with a moderate drop in accuracy on deterministic expressions. Although the accuracy is relatively low on stochastic expressions, one must keep in mind that the task is extremely hard.

In Tab.~\ref{tab:random-leaves-examples}, we show a few examples of expressions that our model succeeded in predicting, showing its remakable ability to isolate the deterministic from the stochastic part. Additionally, our model is able to tell the subtle difference between  $\arctan(\xi)$ and $\sin(\xi)$, which is remarkable: both expressions are random variables with zero mean and very close variance (0.45 and 0.43). 

\begin{table}[htb]
    \centering
    \begin{tabular}{c|c|c}
    \toprule
        $\pi_{train/test}$ & 0 random leaf & 1 random leaf \\
        \midrule
        $\pi_{train}=0$      & \textbf{75.8} & 2.4 \\
        $\pi_{train}=0.1$    & 72.0 & \textbf{17.1} \\        
    \bottomrule
    \end{tabular}
    \caption{\textbf{Our model can be made robust to noise in the sequences, but this lowers performance in absence of noise.} $\pi_{train}$ is the probability to sample a random leaf at training time, and we show the evaluation accuracy at $n_{pred}=10$ and $\tau=10^{-10}$ for expressions with 0 and 1 random leafs. In order to make the problem easier we considered long sequences ($l_{min}=l_{max}=30$) with up to $o_{max}=5$ operators.}
    \label{tab:random-leaves}
\end{table}

\begin{table}[htb]
    \centering
    \begin{tabular}{c|c|c}
    \toprule
    Expression & First guess & Second guess \\
    \midrule
    $\sin(\xi)$ & Correct & $\cos(\xi)$\\
    $\arctan(\xi)$ & Correct & $\arctan(2\xi)$\\
    $u_{n-1}+u_{n-2}+\xi$ & Correct & $u_{n-1}+u_{n-2}+|\xi|$\\
    \bottomrule
    \end{tabular}
    \caption{\textbf{A few non-deterministic functions our model was able to recognize.}}
    \label{tab:random-leaves-examples}
\end{table}

\section{Extension to multidimensional sequences}
\label{app:multidim}

As a proof-of-concept, we show that our method can easily be generalized to multidimensional sequences, with interdependent dimensions.

\paragraph{Method} 
The multidimensional setup deals with systems of $d$ sequences with interdependent expressions. An example for $d=2$ would be $\{u_{n+1} = v_n+1, v_{n+1}=2u_n\}$. We encode this multidimensional expression as a concatenation of the $d$ expressions, separated by a special delimitation token \texttt{del}: [\texttt{sum, v0, 1, del, mul, u0, 2}]. As for the series presented to the model, they are encoded as alternated terms, e.g. [$u_0, v_0, u_1, v_1, ...$].

Because of this encoding, the average length of the input sequences is multiplied by a factor of $d$, which significantly slows down our model due to the quadratic complexity of self-attention in input size. Hence, we restrict ourselves to $d\in\{1,2,3\}$ as a proof of concept.

\paragraph{Results}

In Fig.~\ref{fig:multidim}, we show similar results as before but investigating the 2 and 3 dimensional setup. We observe that in two dimensions, our symbolic model still performs better than the numeric model at high precision and high prediction length. However, the three dimensional setup favors the numeric

\begin{figure*}[htb]
    \centering
    \includegraphics[width=\columnwidth]{figs/acc_vs_difficulty_float_multidim.pdf}
    \caption{\textbf{Our model can handle multidimensional sequences.}}
    \label{fig:multidim}
\end{figure*}

